Campfire: Compressible, Regularization-Free, Structured Sparse Training for Hardware Accelerators

This paper studies structured sparse training of CNNs with a gradual pruning technique that leads to fixed, sparse weight matrices after a set number of epochs. We simplify the structure of the enforced sparsity so that it reduces overhead caused by regularization. The proposed training methodology Campfire explores pruning at granularities within a convolutional kernel and filter. We study various tradeoffs with respect to pruning duration, level of sparsity, and learning rate configuration. We show that our method creates a sparse version of ResNet-50 and ResNet-50 v1.5 on full ImageNet while remaining within a negligible <1% margin of accuracy loss. To ensure that this type of sparse training does not harm the robustness of the network, we also demonstrate how the network behaves in the presence of adversarial attacks. Our results show that with 70% target sparsity, over 75% top-1 accuracy is achievable.

==> Figures.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}
% 3X3 CONVOLUTION PRUNED
\def\xshift{0}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \\
            |[fill=white!30]| \& |[fill=red!30]| \& |[fill=Random\Random!30]|\\
            |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 4) %shift the matrix
        {
            |[fill=white!30]|  \& |[fill=Random\Random!30]| \& |[fill=red!30]| \\
            |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
            |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mb\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 6) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=white!30]| \& |[fill=Random\Random!30]| \\
            |[fill=red!30]| \& |[fill=red!30]| \& |[fill=red!30]|\\
            |[fill=white!30]| \&|[fill=red!30]|  \&|[fill=white!30]| \\
        };
    
}
% \node [below= of mb3.south] (nodeanchor) {}
\node [below= of mb3.south] (lm) {3x3 Conv Sparsity};

% 3x3 CK CONVOLUTION PRUNED
\def\xshift{3.5}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 4 ) %shift the matrix
        {
            |[fill=Random
            \Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mr\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 6 ) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
    
}
\node [right= of lm] (lm) {CK Sparsity};

% 1x1 CONVOLUTION PRUNED
\def\xshift{6.75}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
           |[fill=Random\Random!30]|  \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew+ \xshift, -\x * \ys - 4) %shift the matrix
        {
            |[fill=Random\Random!30]|  \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (ma\x)%give the matrix a name
        at(-\x * \xs + \xnew+ \xshift, -\x * \ys - 6) %shift the matrix
        {
            |[fill=Random\Random!30]|  \\
        };
    
}
\node [right= of lm] (lm) {1x1 Conv Sparsity};

% FULLY CONNECTED PRUNED
\def\xshift{9.3}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\matrix [minimum size=2mm,
         matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
         column sep=-\pgflinewidth, row sep=-\pgflinewidth,
         ampersand replacement=\&] %see explanation
(mfc)%give the matrix a name
at(\xnew + \xshift, -4.75) %shift the matrix
{
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \&
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \\
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \\
        |[fill=white!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \&
    |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \\
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=white!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \\
};
\node [right= of lm] (lm) {FC Sparsity};

% FULLY CONNECTED BLOCK PRUNED
\def\xshift{12.5}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\matrix [minimum size=2mm,
         matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
         column sep=-\pgflinewidth, row sep=-\pgflinewidth,
         ampersand replacement=\&] %see explanation
(mfc)%give the matrix a name
at(\xnew + \xshift, -4.75) %shift the matrix
{
    |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \&
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=red!30]|  \&|[fill=white!30]| \&
    |[fill=white!30]|  \& |[fill=white!30]| \& |[fill=white!30]| \\
    |[fill=red!30]| \& |[fill=red!30]| \& |[fill=white!30]|\&
    |[fill=white!30]| \&|[fill=red!30]|  \&|[fill=red!30]| \\
        |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=red!30]|\\
    |[fill=white!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \&
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=white!30]| \\
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=red!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \\
};
\node [right= of lm] (lm) {FC Block Sparsity};
\end{tikzpicture}
\caption{There are five types of pruning we attempt in this work. Each pruning technique involves either a different layer of the network or a different dimension within the layer of the network. In the figures above, red values represent that weight is zero in the tensor. 
3x3 Conv Sparsity implies that convolutional kernels in 3x3 Conv layers retain only 4 or 2 nonzero values out of 9 values in each kernel after last epoch of pruning. 
CK Sparsity refers to pruning entire kernels in a 3x3 convolutional layer. To do this, we sum the absolute vaues of the weights in the kernel and compare to the absolute sums of all the other kernels. 
1x1 Conv Sparsity implies that the smallest weights in the entire layer are pruned, which applies to 1x1 Convolutional layers. 
FC Sparsity refers to pruning the individual weights in the entire FC Layer, where we compare the magnitude of all the weights to each other. 
FC Block Sparsity implies that we prune an entire 2x2, 3x3 or 4x4 window within the FC layer, which creates a coarser grained sparsity. To do this, we sum the magnitude of the weights in each window and prune the windows with the smallest magnitude.} 
\label{fig:3x3convprune}
\end{figure}

==> Sparsity Paper (2)/Abstract.tex <==
\vspace{-10pt}
\begin{abstract}
This paper studies structured sparse training of CNNs with a gradual pruning technique that leads to fixed, sparse weight matrices after a set number of epochs. 
We simplify the structure of the enforced sparsity so that it reduces overhead caused by regularization.
The proposed training methodology Campfire explores pruning at granularities within a convolutional kernel and filter.

We study various tradeoffs with respect to pruning duration, level of sparsity, and learning rate configuration.
We show that our method creates a sparse version of ResNet-50 and ResNet-50 v1.5 on full ImageNet while remaining within a negligible $<$1\% margin of accuracy loss.
To ensure that this type of sparse training does not harm the robustness of the network, we also demonstrate how the network behaves in the presence of adversarial attacks.  Our results show that with 70\% target sparsity, over 75\% top-1 accuracy is achievable.
\end{abstract}

% keywords can be removed

%\keywords{Deep learning \and Sparsity \and Architecture \and Adversarial \and Regularization-Free \and Convolutional Neural Network \and ResNet \and Imagenet}

==> Sparsity Paper (2)/Acknowledge.tex <==
\subsubsection*{Acknowledgments}
We thank Vitaliy Chiley, Sara O'Connell, Xin Wang, and Ilya Sharapov for their feedback on the manuscript.
This research was sponsored by NSF grants
CCF-1563113. Any opinions, findings and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation (NSF).


==> Sparsity Paper (2)/Conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

In this work, we introduced techniques to train CNNs with structured sparsity and studied the tradeoffs associated with various implementation options. We demonstrated on ResNet-50 with the full ImageNet dataset that the proposed sparse training method outperforms all related work and is comparable to a dense model in terms of convergence accuracy. %We also observed that the early stages (0-30 epochs) of dense training are critical for reaching high convergence accuracy.
We also observed that delaying the start of enforced, gradual pruning to at least epoch 20 was necessary to reach high convergence accuracy, highlighting the importance of the early epochs of dense training. 
Moreover, performing an additional 10 epochs of training provides substantial (around 1\%) accuracy gains of the final model.
In the future, we would like to study the tradeoffs of sparse training on low-precision networks.


==> Sparsity Paper (2)/Experiments.tex <==
\section{Experimental Setup}
\label{sec:setup}

To validate each type of pruning (window, CK, or combined) we selected ResNet-50 \cite{resnet50} v1 and v1.5 with the ImageNet and/or Tiny-ImageNet \cite{tinyimagenet} datasets. We evaluated each pruning method by varying \textit{sparsity levels} and \textit{pruning era}. Smaller batch (64) experiments were each run on one NVIDIA RTX 2080 GPU, and larger batch (256) experiments were run on 4. Each network was implemented in PyTorch \footnote{\url{https://pytorch.org/}}.

We experimented with ResNet-50 v1.5, in addition to v1, to explore how changing the network structure would affect the top-1 accuracy. For window pruning, we tested with ResNet-50 v1 on Tiny-ImageNet as well as ResNet50 v1 and v1.5 on ImageNet to compare the impact of strided convolutions on our sparse training.
Also, we experimented with the learning rate schedule of the training regime. Our typical  schedule for ResNet-50 v1.5 included learning rate drops at epochs 30, 60, and 90, but we experimented with placing the last drop at epoch 80 instead. 
For the majority of our experiments, we used batch size 64 as this is what could fit in one of our GPUs. As suggested by Krizhevsky \cite{krizhevsky2014weird}, we scaled the starting learning rate by $\frac{1}{\sqrt{4}} = \frac{1}{2}$ to 0.05 in order to compensate for the smaller batch size. We also showed results with batch size 256 spread across 4 GPUs and starting the learning rate at 0.1.


%We define each testing domain below in section \ref{sec:experiments_domains}. We define the experiments applied to these domains in section \ref{sec:experiments_pruning}

%\TODO{We can move this entire subsection on domains to the appendix}
%\subsection{Models and Dataset Domains}\label{sec:experiments_domains}

%Each experiment of the sparsity mechanism ran in a specific test domain designed to represent a standard training environment. We defined each of these domains below and refer to them in Section \ref{sec:experiments_pruning}.

% For our work, we include three different experiment setups. All experiments operate with ResNet-50 on ImageNet in some form. The first experiment involves ResNet-50 v1 on Tiny-ImageNet (a smaller version of ImageNet), the second involves ResNet-50 v1 on ImageNet (ILSVRC2012), and the third involves ResNet-50 v1.5 on ImageNet (ILSVRC2012). 

% The sparsity only changes every epoch

\begin{comment}
\subsubsection{Saved Multiplies Estimate}

In our evaluation, we present the metric \textit{percentage saved multiplies}.
This metric is designed to estimate the percentage of multiplies by zero throughout all of training. 
We felt that knowing this metric was important because it is an indicator of saved energy as well as shows the potential of how many multiply operations we can remove if we were to optimize with hardware. 
In order to estimate this value, we first determine the number of Multiply-Accumulate operations that occur per layer in ResNet-50. 
With pytorch, we can perform this with hooks and there are many online implementations to validate our calculations, such as \footnote{\url{https://github.com/ceykmc/pytorch_model_summary}}. 
We use the following equation to estimate percentage saved multiplies (psm):
\begin{align*}
    \mathrm{psm} = \frac{ \sum_{i=1}^{n} \mathrm{spt}_i \times \mathrm{tma}_p} {n \times \mathrm{tma}_f }
\end{align*}
where \(\text{spt}_i\) is the amount of sparsity at epoch \(i\) of training and \(n\) is the number of epochs of training. \(\text{tma}_p\) is the total number of prunable multiplies (all the multiplies from convolutions and linear layers and not batch norm, pooling, and activations). \(text{tma}_f\) is the total number of multiplies in the network, including all batch norm, pooling and activation layers. 
\end{comment}

\subsection{Sparse Training Experiments}

Tiny-Imagenet, which has 100,000 training images~\cite{tinyimagenet}, is an easier task than full ImageNet (1.2 million images~\cite{imagenet}), but it takes less time to train and is still somewhat predictive of performance on ImageNet as it contains the same type of images. Accordingly, we ran with Tiny-Imagenet on ResNet-50 v1 as a preliminary test of our pruning methods. As dense training with this benchmark only requires 40 epochs to converge and we wanted to fix the sparsity mask as early in the training as possible, we used a pruning era of epochs 0-10. Early experiments showed this to be sufficient to achieve full accuracy with Window and CK pruning.
%We subsequently enforced the final sparsity requirement, set a maximum number of non-zero values in each window/kernel of each layer, and fixed this sparsity pattern for the rest of training. We chose the 10th epoch as the \textit{final epoch of pruning} because we wanted to see if we could fix the sparsity mask early in the training process. 
%For the ResNet-50 v1 and Tiny-ImageNet, we ran the gradual pruning mechanism until the 10th epoch of training while not enforcing a max number of nonzeros in the network and any values could become sparse. After the 10th epoch, we enforce the final sparsity requirement as well as the setting a number of maxnonzero values in windows of each layer and fix this sparsity pattern for the rest of training. We chose the 10th epoch as the \textit{final epoch of pruning} because we wanted to see if we could fix the sparsity mask early in the training process. Since we are pruning each layer to the specified sparsity value and then enforce the maxnonzero values on the network after the 10th epoch, there are jumps in the sparsity levels. 

In order to find the ideal pruning era and compare the relative performance of our pruning methods (Window, CK, and Combined), we mainly used ResNet-50 v1 and ResNet-50 v1.5 with ImageNet. As trying every permutation of pruning era length and starting epoch was infeasible for us resource-wise, we used our early experiments to guide our search. Initially, with window and CK pruning we experimented with pruning at the beginning of training (epochs 0-30). While these experiments were promising with Window pruning, CK pruning was not effective early in training. Furthermore, we tried a shorter \textit{pruning era} (0-20) with Window but found this caused a large drop in accuracy, so we mostly moved away from pruning in the early epochs. 

Next, we hypothesized that epoch 30 would be a suitable epoch to stop pruning as this is the epoch of the first learning rate decrease. Results with all methods using a pruning era of 30-50 were promising, so we searched around starting epoch 30. Accordingly, we adopted a similar approach to Han et al. \cite{han2015learning} to train with all pruning methods by setting the \textit{first epoch of pruning} to 20, 30, or 40 and the \textit{pruning era} to 20 or 30 epochs. In these combinations, we experimented with the following sparsities (and report the most important results): 20, 40, 60, 70, 80, and 90\%.

We did experiment with earlier starting epochs (10, 15) and a shorter pruning era lengths (10); however, these caused large losses in accuracy, so we did not pursue them fully. We did not pursue later starting epochs or longer pruning eras because our goal was to fix the sparsity mask early and prune for as few epochs as possible.

%For ResNet50 v1 and ImageNet, our goal was to start pruning as early as possible, while maintaining high accuracy. We set our \textit{pruning era} to epochs 0-30. Our hypothesis was that 30th epoch would be a suitable epoch to stop pruning, because this is where the learning rate is first decreased. In addition, there would be a large drop in accuracy if we stop pruning at epoch 20. However, this schedule did not perform well for ResNet-50 v1.5 and ImageNet and therefore we set our \textit{pruning era} to 30-50.

%Our initial experiments found this was a suitable epoch to stop pruning because this was where the learning rate was first decreased, in addition, there was a large drop in accuracy if we stopped pruning at epoch 20. As a result, when we found for ResNet5-0 v1.5 and ImageNet setting the \textit{pruning era} to epochs 0-30 did not perform well, we also tried 30-50. 

%To test training using CK and combined pruning, we mainly used ResNet-50 v1 and ResNet-50 v1.5 with ImageNet, but also performed CK pruning on ResNet-50 v1 and Tiny-ImageNet. We adopted a similar approach to \cite{han2015learning} to train with CK or combined pruning by setting the \textit{first epoch of pruning} to 20, 30, or 40 with a \textit{pruning era} of 20 or 30 epochs. Then, we continued to train the sparsified network until the final epoch. 

In each of network/dataset combinations, we compare to a densely trained baseline and other works of literature that performed corresponding experiments.

\subsection{Adversarial Robustness}

Since there was evidence that increasing sparsity lowers adversarial robustness \cite{wang2018adv}, we evaluated this robustness in our models.
To do so, we applied \textit{Fast Gradient Sign Method} (FGSM) attacks \cite{goodfellow2014explaining} on one of our sparse models, to generate its own adversarial examples, and measured the validation accuracy again. 
We used the same validation set as ImageNet and applied the attack's image transformation to each input image.
Moreover, we experimented with a variety of different \(\epsilon\) in order to see how our accuracy decayed. 
Lastly, in our experiments we leveraged the examples provided in Pytorch tutorials. \footnote{\url{https://pytorch.org/tutorials/beginner/fgsm_tutorial.html}}
%Lastly, we leveraged the implementation details provided by \footnote{\url{https://pytorch.org/tutorials/beginner/fgsm_tutorial.html}}.

\begin{comment}
\subsection{PRISM Platform}

\NJG{For \TODO{Anand}:
\begin{itemize}
\item Can you fill in ALL of the relevant dependencies for PRISM? 
\item Why did pytorch make sense? \item What makes it different from other frameworks? 
\item And what does it build on from other frameworks (ie Intel's Distiller)? 
\item Mostly like what was happening at the beginning of this project. Shouldn't be more than few sentences. 
\end{itemize}
}

To rapidly prototype strategies and test across network types, we developed our own platform called PRISM using PyTorch; the custom operations were defined as individual \texttt{nn.Module}s. PRISM enables users to configure their runs in a single configuration file and the platform will run that experiment. It logs all the data from the run in order to effectively analyse the model. In addition to supporting different sparsity mechanisms, the platform supports reduced precision training and regularization techniques as well. 
We've since learned about equivalent and independent effort by Intel AI group the Neural Network Distiller ~\cite{NNDistiller}. 
\end{comment}



==> Sparsity Paper (2)/Figures.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}
% 3X3 CONVOLUTION PRUNED
\def\xshift{0}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \\
            |[fill=white!30]| \& |[fill=red!30]| \& |[fill=Random\Random!30]|\\
            |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 4) %shift the matrix
        {
            |[fill=white!30]|  \& |[fill=Random\Random!30]| \& |[fill=red!30]| \\
            |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
            |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mb\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 6) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=white!30]| \& |[fill=Random\Random!30]| \\
            |[fill=red!30]| \& |[fill=red!30]| \& |[fill=red!30]|\\
            |[fill=white!30]| \&|[fill=red!30]|  \&|[fill=white!30]| \\
        };
    
}
% \node [below= of mb3.south] (nodeanchor) {}
\node [below= of mb3.south] (lm) {3x3 Conv Sparsity};

% 3x3 CK CONVOLUTION PRUNED
\def\xshift{3.5}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 4 ) %shift the matrix
        {
            |[fill=Random
            \Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
                %draw, % for the rectangle border
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mr\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 6 ) %shift the matrix
        {
            |[fill=Random\Random!30]|  \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \\
            |[fill=Random\Random!30]| \& |[fill=Random\Random!30]| \& |[fill=Random\Random!30]|\\
            |[fill=Random\Random!30]| \&|[fill=Random\Random!30]|  \&|[fill=Random\Random!30]| \\
        };
    
}
\node [right= of lm] (lm) {CK Sparsity};

% 1x1 CONVOLUTION PRUNED
\def\xshift{6.75}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\foreach \x in {1,2,...,\nm}
{
        %draw, % for the rectangle border
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mp\x)%give the matrix a name
        at(-\x * \xs + \xnew + \xshift, -\x * \ys - 2) %shift the matrix
        {
           |[fill=Random\Random!30]|  \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (mq\x)%give the matrix a name
        at(-\x * \xs + \xnew+ \xshift, -\x * \ys - 4) %shift the matrix
        {
            |[fill=Random\Random!30]|  \\
        };
        \pgfmathsetmacro\Random{random(0,1)}
        \matrix [minimum size=2mm,
                 matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
                 column sep=-\pgflinewidth, row sep=-\pgflinewidth,
                 ampersand replacement=\&] %see explanation
        (ma\x)%give the matrix a name
        at(-\x * \xs + \xnew+ \xshift, -\x * \ys - 6) %shift the matrix
        {
            |[fill=Random\Random!30]|  \\
        };
    
}
\node [right= of lm] (lm) {1x1 Conv Sparsity};

% FULLY CONNECTED PRUNED
\def\xshift{9.3}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\matrix [minimum size=2mm,
         matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
         column sep=-\pgflinewidth, row sep=-\pgflinewidth,
         ampersand replacement=\&] %see explanation
(mfc)%give the matrix a name
at(\xnew + \xshift, -4.75) %shift the matrix
{
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \&
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \\
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \\
        |[fill=white!30]|  \& |[fill=white!30]| \& |[fill=red!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \&
    |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \\
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=white!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \\
};
\node [right= of lm] (lm) {FC Sparsity};

% FULLY CONNECTED BLOCK PRUNED
\def\xshift{12.5}
\def\xs{.25} %shift in x direction
\def\ys{0.25} %shift in y direction
\def\nm{5} % number of 2d matrices in the 3d matrix
\def\xnew{2}
\colorlet{Random0}{white}
\colorlet{Random1}{red}
\pgfmathsetmacro\Random{random(0,1)}
\matrix [minimum size=2mm,
         matrix of nodes, nodes={draw, outer sep=0pt},nodes in empty cells,
         column sep=-\pgflinewidth, row sep=-\pgflinewidth,
         ampersand replacement=\&] %see explanation
(mfc)%give the matrix a name
at(\xnew + \xshift, -4.75) %shift the matrix
{
    |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \&
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=white!30]|\\
    |[fill=red!30]| \&|[fill=red!30]|  \&|[fill=white!30]| \&
    |[fill=white!30]|  \& |[fill=white!30]| \& |[fill=white!30]| \\
    |[fill=red!30]| \& |[fill=red!30]| \& |[fill=white!30]|\&
    |[fill=white!30]| \&|[fill=red!30]|  \&|[fill=red!30]| \\
        |[fill=red!30]|  \& |[fill=red!30]| \& |[fill=white!30]| \&
    |[fill=white!30]| \& |[fill=red!30]| \& |[fill=red!30]|\\
    |[fill=white!30]| \&|[fill=white!30]|  \&|[fill=red!30]| \&
    |[fill=red!30]|  \& |[fill=white!30]| \& |[fill=white!30]| \\
    |[fill=white!30]| \& |[fill=white!30]| \& |[fill=red!30]|\&
    |[fill=red!30]| \&|[fill=white!30]|  \&|[fill=white!30]| \\
};
\node [right= of lm] (lm) {FC Block Sparsity};
\end{tikzpicture}
\caption{There are five types of pruning we attempt in this work. Each pruning technique involves either a different layer of the network or a different dimension within the layer of the network. In the figures above, red values represent that weight is zero in the tensor. 
3x3 Conv Sparsity implies that convolutional kernels in 3x3 Conv layers retain only 4 or 2 nonzero values out of 9 values in each kernel after last epoch of pruning. 
CK Sparsity refers to pruning entire kernels in a 3x3 convolutional layer. To do this, we sum the absolute vaues of the weights in the kernel and compare to the absolute sums of all the other kernels. 
1x1 Conv Sparsity implies that the smallest weights in the entire layer are pruned, which applies to 1x1 Convolutional layers. 
FC Sparsity refers to pruning the individual weights in the entire FC Layer, where we compare the magnitude of all the weights to each other. 
FC Block Sparsity implies that we prune an entire 2x2, 3x3 or 4x4 window within the FC layer, which creates a coarser grained sparsity. To do this, we sum the magnitude of the weights in each window and prune the windows with the smallest magnitude.} 
\label{fig:3x3convprune}
\end{figure}

==> Sparsity Paper (2)/Intro.tex <==
\section{Introduction}
\label{sec:intro}

Pruning weights can compress a neural network into a smaller model that can fit into faster/smaller memory and therefore result in execution speedups \cite{EIE, han2015deep}. To increase the accuracy of sparse models, Han et al. \cite{han2015learning} and Mao et al. \cite{mao2017exploring} explore training the network dense after pruning.
The resulting network can maintain accuracy based on the specified level of sparsity~\cite{mostafa2019parameter, topruneornot, han2015deep}.

Structured sparsity, where a certain number of non-zeros is allowed across various cross-sections of the weight tensors, has been explored for RNNs and also CNNs. These methods aim to speed up computation and reach some final level of sparsity for deployment. Narang et al. \cite{narang2017exploring} have shown promising results for structured training of RNNs while sparse CNNs could not achieve the same performance \cite{mao2017exploring}.

Recent work has demonstrated that structurally-sparse training can speed up execution on GPUs~\cite{he2017channel, prunetrain, topruneornot}.
However, these training mechanisms add regularization (and thus computational overhead) to eliminate unnecessary weights. 
Regularization includes operations such as norm \cite{grouplasso}, involving division and square root, which are expensive for ASIC accelerators as they are atypical and high latency \cite{wu2018l1}.
%The regularization term modifies the original training and can be expensive in hardware. 
While enforcing coarse-grain sparsity, PruneTrain \cite{prunetrain} provides significant speedups, but the final network contains a low degree of sparsity. Higher sparsity levels are necessary to offset the overheads incurred by indexing/compression/decompression \cite{kourtis2010data} and to fit models on memory-limited platforms such as mobile or embedded devices \cite{lin2019toward}.

Mostafa and Wang \cite{mostafa2019parameter} show that with adaptive sparse training and dynamic reallocation of non-zeros sparsity levels up to {80\%} can be achieved. However, to achieve an accuracy loss of 1.6\% an additional 10 epochs (100 total compared to the typical 90 epochs) of training are required. The main drawback is the overhead incurred while implementing such a technique on the target platform.
Continuous reconfiguration of the sparsity pattern is expensive in hardware as creating a compressed format is memory-intensive and energy-inefficient \cite{pedram2016dark}. Restructuring the sparsity pattern frequently requires recompression of data. The incurred memory accesses overshadow the savings when skipping computations with zeros and thus makes weight compression infeasible.
%as it does not allow for compression of weights during training. 
%Continuous reconfiguration of the sparsity pattern is expensive as it does not allow for compression of weights during training. 
%Creating a compressed format is a memory-intensive operation in the hardware, which is very energy inefficient(cite dark memory). 
%Restructuring the sparsity pattern frequently requires recompression of data. The incurred memory accesses overshadow the savings when skipping computations with zeros.

Our goal is to provide high levels of sparsity (>60\%) during training with minimal degradation of accuracy. Additionally, to make our training more memory-efficient and accelerator-friendly, we seek to make the sparsity structured, to remove irregular computations like regularization, and to avoid decompression/recompression at each training step. Our main motivating insight is that having a \textit{fixed} sparse multiply-accumulate pattern allows weight compression during training and can save compute and energy in hardware \cite{EIE}.

To achieve our goal, we introduce Campfire, a sparse training method that applies the techniques in Han et al. \cite{han2015learning} and Mao et al. \cite{mao2017exploring} at earlier stages in training within what we call the pruning era, usually a period of 20-30 epochs.
%Assuming a convolution layer has tensor size $RSCK$. $R$ and $S$ are the convolution kernel height and width, and $C$ and $K$ are the input and output number of channels respectively.
During the pruning era, we exploit one of the three proposed sparsity regimes, which have granularities of at most a whole kernel, to prune the network.
After this period, we fix the sparsity mask for the rest of the training. 
Since sparsification reduces the total number of computations \cite{zhu2019sparse, parashar2017scnn} and hardware accelerators have mechanisms to skip computations with zeros \cite{han2015learning}, fixing the mask early in training results in speedups and thus makes an earlier shorter pruning era ideal.
We seek to find this ideal pruning era by characterizing different combinations of pruning era length and start epoch with our original goal of high sparsity and high accuracy in mind.

As such, we explore the impact of various pruning granularities, sparsity levels, and learning-rate schedules on the network's convergence as well as adversarial robustness for CNNs like ResNet-50~\cite{resnet50} on ImageNet and Tiny Imagenet~\cite{tinyimagenet}.

%Our goal for this work is to explore various pruning methodologies with focus towards a regularization free structured pruning mechanism. 

%There is evidence that larger and sparser models can perform better than their smaller yet denser equivalents, given the same number of weights per model \cite{topruneornot}. However, this causes the network to lose efficiency in a target hardware platform as a majority of the multiply accumulate units become zero in the dense kernel but the sparsity pattern is irregular and unpredictable. 

%We settled on the idea of pruning the model for a certain period of less than 20-30 epochs at the beginning of training to get to a satisfying sparsity level. With a fixed sparsity pattern of the weights, training the network can yield in performance improvement in hardware accelerator as there won't be any updates/modifications on the sparsity mask and the resulting indexing of the weights for the remainder of training. We explore different pruning mechanisms that create fixed-sparse models early during training without changing the original training regime. 

Recent literature~\cite{wang2018adv} has shown that adversarial attacks are more successful on pruned neural networks than they are on regular neural networks. 
Given the danger of adversarial attacks in real world situations, we find that it is important to evaluate our sparsity techniques under adversarial robustness. 
We leverage the FGSM mechanism~\cite{goodfellow2014explaining} to evaluate the adversarial robustness on our sparse models.
This paper makes the following contributions:
\begin{enumerate}
     \item  We propose a mechanism to train and prune a convolutional network during the earlier stages of training such that this sparsity can be harvested for the computational speedups. To do this, we fix the sparse weight masks for the remainder of the training. %Our pruning period only lasts for 20-30 epochs of training.
     \item For fully connected sparsification, we eliminate blocks of fully connected weights based on their connection to the zeros in the previous convolutional layer.
      \item We enforce structural, regularization free, magnitude-based pruning across two distinct dimensions and a combined version. These dimensions are inside convolution window $R \times S$ and across input/output feature matrix ($CK$).
    %\item Our results demonstrate that a pruning mechanism which requires negligible modification in the training regime can achieve within .13\% standard model accuracy ResNet-50 on full Imagenet after the same number of epochs and overall fewer multiplications in training.
    \item Our sparse models are as robust to adversarial FGSM attacks as fully dense models. 
    %\item We find that with our mechanism, we can achieve accuracy degradation of 0.13\% (74.8\% top1 accuracy) with 60\% of the values in the network set to zero after 30th epoch of training for ResNet-50 on Imagenet and maintain roughly the same level of adversarial robustness.
    \item We demonstrate that early stage dense training is crucial for maintaining high accuracy.
    
    \item The proposed technique is tolerant to sparsity levels of up to 60-70\% with under 1\% accuracy degradation. We can compensate by scheduling an extra learning rate drop and training for an extra 10 epochs.

\end{enumerate}


The rest of the paper is organized as follows. Section~\ref{sec:methodology} explains our pruning methodology. Section~\ref{sec:setup} describes the experimental setup framework. Section~\ref{sec:results} presents results and discusses their interpretation. Section~\ref{sec:related} presents the related work. Section~\ref{sec:conclusion} concludes the paper.
% \begin{enumerate}
    % \item \AP{ Noah, please add some bullets about why pruning is important in training and what is missing today}
    % \item the goal is to show that you can prune models in a way that makes them amenable to building custom hardware for training them.
    % \item You can train really huge models sparsely, which has been shown to get better accuracy
    % \item Gradual pruning technique applied Leads to a sparse network 
    % \item Our goal is to explore how we can prune in a hardware-sensitive way \AP{what has been done so far?}
    % \item 
    % \item in hardware we want to make use of sparse weights easy for the forward pass
    % \item in hardware we want to make sparse weight updates also easy (need to elaborate on this)
    % \item in hardware storing weights in sparse fashion creates levels of indirection which is expensive.
    % \item here we have to emphasize the focus of this space is to push for studying sparsity mainly on the network side and designing hardware is out of the focus of this paper
    % \item We use the pruning mechanism shown in \cite{topruneornot}. \AP{Then what was is our contribution ?}
    % \item The constributions of this paper are as follows:
    % \item \TODO{Contribution \#1}
    % \item \TODO{Contribution \#2}
    % \item \TODO{Contribution \#3}

% \end{enumerate}


==> Sparsity Paper (2)/Pruning.tex <==

\section{Pruning Methodology}
\label{sec:methodology}

\begin{comment}
\begin{figure}[H]
    \centering
    \includegraphics[width=.30\textwidth]{Figures/pruning_pic.pdf}
    \caption{This represents our general sparsity mechanism}
    \label{fig:pruning_methodology}
\end{figure}
\end{comment}

\begin{figure}[t]
   \vspace{0pt}
   \centering
        \begin{subfigure}[b]{0.22\textwidth}
           \includegraphics[width=\textwidth]{Figures/pruning_pic.pdf}
           \caption{}
           \label{fig:chart}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.75\textwidth}
           \includegraphics[width=\textwidth]{Figures/pruning_era.pdf}
          \caption{}
           \label{fig:timing}
        \end{subfigure}

\vspace{-10pt}
\caption{(a) Our general sparsity mechanism in which we update the sparsity mask after each batch until we reach a desired level of sparsity. (b) Schedule comparison between this work, Mostafa ang Wang \cite{mostafa2019parameter}, and PruneTrain \cite{prunetrain}. Our work has the shortest pruning era and more gradually reaches our final sparsity. }
\label{fig:pruning_methodology}
\end{figure}


Our proposed pruning mechanism works by always pruning the weights of smallest magnitude after each weight update. After a forward and backward pass (one batch update), the model is pruned. If a weight is already zero, the gradient is also set to zero. This means that once a weight becomes zero, it will remain zero for the rest of the training period. 

This mechanism is similar to Han et al. \cite{han2015learning}, except that we only prune in the earlier stages of the training as opposed to post training. 
Additionally, this work is similar to Narang et al. \cite{narang2017exploring} although we set the sparsity threshold instead of using a heuristic to calculate it.
We chose this pruning mechanism because of its negligible computational overhead. 


In our pruning algorithm, %presented in detail in Algorithm~\ref{alg:pruning_method},
%the \textit{first epoch of pruning} refers to the training epoch where we start pruning the network weights.
the sparsity threshold refers to the percentage of weights in the network that are currently pruned. Before or during the first epoch of pruning, we will have a sparsity threshold of zero. 
As we continue training, we gradually increase the sparsity threshold so that by the final epoch of pruning the network sparsity will have reached our final, desired threshold.
This gradual increase is achieved by setting the threshold as shown in the following equation in each epoch within the pruning window:
\begin{align}
    \text{sparsity\_threshold} = s_f - (s_i + s_f) (1 - \frac{e_c - e_i}{l_p})^r
\end{align}
Where $s_f$ is the final desired sparsity, $s_i$ is the initial sparsity (always 0 in our case), $e_c$ is the current epoch, $e_i$ is the initial epoch of pruning, $l_p$ is the length of the \textit{pruning era}, and $r$ controls how fast or slow the threshold increases exponentially  (in our case $r=3$).

We define the \textit{pruning era} to be the epochs between the first and final epochs of pruning depicted in Figure~\ref{fig:timing}.

Finally, we evaluate the pruning mask after every training step until we reach the final epoch of pruning. After the final epoch, the pruned values in the network will remain zero for the rest of training; no new pruning will occur, and only the non-zero weights will be updated. %During training, we ensure we prune the gradient updates of the last updated value. We do this so that any hardware could exploit this fixed sparsity pattern.


\begin{figure}[t]
   \vspace{0pt}
   \centering
        \begin{subfigure}[b]{0.31\textwidth}
           \includegraphics[width=\textwidth]{Figures/Window_sp.pdf}
           \caption{}
           \label{fig:window_pruning}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.3\textwidth}
           \includegraphics[width=\textwidth]{Figures/CK_Sp.pdf}
          \caption{}
           \label{fig:ck_pruning}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.15\textwidth}
          \includegraphics{Figures/FC_sp.pdf}
          \caption{}
           \label{fig:fc_pruning}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.15\textwidth}
          \includegraphics{Figures/FC_Blk.pdf}
          \caption{}
           \label{fig:block_fc_pruning}
        \end{subfigure}
 \vspace{-10pt}
 \caption{
This figure illustrates sparsity across different weight dimensions and different granularities. (a) \textit{Window sparsity}, which prunes the 5 smallest weights in a 3$\times$3 window. (b)\textit{CK pruning} where whole R$\times$S convolutional kernels are pruned. (c) Sparsity in fully-connected weights. (d) Block sparsity in a fully-connected layer.}

%Examples of different pruned weight tensors.  Each pruning technique we use involves either a different layer of the network or a different dimension within the layer of the network. Figures~\ref{fig:window_pruning},\ref{fig:ck_pruning} represent to the weight tensor of a 3x3 convolutional layers. Figures~\ref{fig:1x1_window_pruning} represent the weight tensor of a 1x1 convolutional layer. Figurers~\ref{fig:fc_pruning},\ref{fig:block_fc_pruning} represent the weight tensors of dense layers. In each tensor above, red squares represent that the corresponding weight is zero in the tensor and white squares represent that the corresponding weight is non-zero } 
\label{fig:3x3convprune}
\vspace{0pt}
\end{figure}


\subsection{Pruning Methodology by Layer}
\label{sec:layer-pruning}

Pruning the smallest magnitude weights in the \textit{entire} network is inefficient because it involves sorting the weights over the network. Instead, we prune the smallest magnitude weights or sum of weights, within a certain locale of the network. When pruning, we examine each layer individually and apply a separate technique to evaluate which weights to prune, depending on the type of layer we are currently pruning. 

\begin{comment}
The model we use for our evaluation is ResNet-50~\cite{resnet50}. This model consists of 3x3 convolutions, 1x1 convolutions, and a fully connected layer. Our pruning mechanism is designed to efficiently prune these different kinds of layers. To see how we prune each of these layers in their own way please see Figure~\ref{fig:3x3convprune}. 
\end{comment}

\subsubsection{Convolutional Layer Pruning}



\paragraph{Window pruning for 3x3 Convolutional Layers}
Figure~\ref{fig:window_pruning} shows the result of a pruned 3$\times$3 convolutional weight tensor under the window pruning method. 
In this scheme, window layer pruning refers to pruning of weights within the 3$\times$3 convolution kernels. 
%As shown in Algorithm~\ref{alg:window_pruning},
We allow a maximum number of non-zero values for each kernel in the 3$\times$3 convolutional layers and eliminate the weights of smallest magnitude. We set this fixed value so that a hardware accelerator could allocate a fixed dataflow based on these maximum values \cite{EIE}.
%This reduces the computation to a fix pre-determined mapping.
%However, this means that when we specify a sparsity value (perhaps 20\%), the overall sparsity of the network may be higher than that because we could set the number of nonzero values in the kernel of the 3x3 convolution to 2 or 4. 

\paragraph{CK Pruning Methodology}

\begin{algorithm}
\footnotesize
\caption{CK Pruning Algorithm}
\label{alg:ck_pruning}
\begin{algorithmic}
\STATE generate\_ck\_sparsity\_mask($\theta_{layer}$, sparsity\_threshold):
    \FOR{$\theta$ in $\theta_{layer}$}
        \FOR{all c in C} 
            \FOR{all k in K}
                \STATE kernel\_max$_{c,k}$ = max($\theta_{c,k}$)
            \ENDFOR
            \STATE cutoff\_index = size($\theta_c$) $*$ sparsity\_threshold
            \STATE n = max(cutoff\_index, size($\theta_c$) $-$
            max\_non\_zero $-$ 1)
            \STATE cutoff\_value = $n^{th}$ largest value in kernel\_max$_c$
            \FOR{all k in K}
                \STATE mask$_{c,k}$ $=$ 1 if kernel\_max$_{c,k}$ $>$ cutoff\_value, else 0
            \ENDFOR
        \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}

Figure~\ref{fig:ck_pruning} shows the result of a pruned 3$\times$3 convolutional weight tensor under the CK pruning method. 
In this scheme, the weights of a certain layer can be viewed as a CK matrix of R$\times$S kernels. 
    %In this scheme, we try to sparsify the CK matrix in which a zero mean a corresponding R$\times$S window is completely zero. 
The CK pruning method involves pruning the 3$\times$3 convolutions along the channel and kernel dimensions of each convolutional filter, i.e., we prune whole kernels (CK matrix of R$\times$S windows) at once and can ultimately prune all the input channels in an output channel. 
As defined by Algorithm~\ref{alg:ck_pruning}, we determine which filter to prune by examining the max of the magnitudes of all the weights in a kernel, which is the max of nine weights. 
This max is used to evaluate whether the whole kernel should be pruned or not.
%Window Pruning for 1$\times$1 convolutional layers is equal to CK pruning.

\paragraph{Combined Pruning Methodology}
To combine window and CK pruning, we introduce a \textit{combined pruning method}.
As shown by appendix Algorithm~\ref{alg:combined_pruning} in the Appendix, in a given epoch we first apply window pruning to each 3$\times$3 convolutional layer at a fraction of the \textit{sparsity threshold} for that epoch. Then, we prune the remaining fraction of the \textit{sparsity threshold} with CK Pruning. Combined pruning has a \textit{window pruning threshold} hyperparameter (between 0 and 1) that determines how much window pruning is done. It is multiplied with the current epoch's sparsity threshold to get a new threshold used for the window pruning phase. We set this parameter to 0.8 in our experiments.
     

\begin{figure}[t]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\textwidth]{Figures/FC_pruning.pdf}
    \vspace{-15pt}
    \caption{FC pruning taking advantage of the sparsity in the previous convolution layer.}
    \vspace{-5pt}
    \label{fig:FC_pruning}
\end{figure}
 
\subsubsection{Fully Connected Pruning}
Like pruning for convolutional layers, we apply a two-tier pruning scheme from Mao et al. \cite{mao2017exploring} for fully connected layers: micro-level pruning within a block and macro-level pruning that eliminates entire blocks. 
%We apply two pruning mechanisms for fully connected layers with the same granularity types as explored in \cite{mao2017exploring}. 

\paragraph{Block  FC Pruning} Figure~\ref{fig:block_fc_pruning} refers to pruning of individual blocks. Here, we prune an entire n$\times$n (n$<$5) window within the dense layer and create coarse grained sparsity. To do this, we sum the magnitude of the weights in each window and prune the windows with the smallest magnitude. 

\paragraph{Fine FC Pruning} Figure~\ref{fig:fc_pruning} refers to the pruning of individual weights. Here, we prune the individual weights in the entire FC Layer, where we compare the magnitude of all the weights to each other. 

The produced zero patterns in the last convolution layer allow for eliminating more weights in fully connected layer as depicted in Figure~\ref{fig:FC_pruning}.  
If all the $C$ windows for a specific $K_i$ are zeros, the output activation for the corresponding $K_i$ is also zero. 
The corresponding neurons in the following fully connected layer are therefore receiving zero input activations and can be eliminated along with their associated weights. 
This enables us to get sparsity without having to evaluate the weights in the fully connected layer. 

When pruning just the small weights in the FC layer, one can inadvertently cut off relevant connections between the input and output layers. Accordingly, we structure the pruning mechanism such that each output neuron should be influenced by the input. This means every column in the weight matrix of the fully connected layer in Figure~\ref{fig:FC_pruning} has at least one non-zero element.

%\subsection{Weight Update Mechanism}

%\begin{enumerate}
%    \item Our pruning mechanism operates after every mini-batch forward and backward pass, up until the last epoch of pruning. 
%    \item The forward and backward pass operate 
%    \item \NJG{Finish weight update mechanism}
%\end{enumerate}
    

==> Sparsity Paper (2)/Related.tex <==
\section{Related Work}
\label{sec:related}

To give a broad comparison stage, we extended Mostafa and Wang's \cite{mostafa2019parameter} table on alternative sparsity mechanisms in Table \ref{tab:sparsity_work} with respect to characteristics of their mechanisms: training/compression focus, regularization, the period in which pruning is applied, strictness of parameter budget, and pruning granularity.
We explain each of the columns below: 

\begin{enumerate}

    \item \textbf{Training Focus}: Trying to train while maintaining/increasing sparsity of the network. The opposite is \textbf{Compression Focus}, i.e., methods that only seek to provide a smaller network for inference.  

    \item \textbf{Regularization}: Applying a regularization value to the loss, in order to find and prune irrelevant weights, while others use magnitude-based pruning.

    \item \textbf{Pruning Era}: The period during training in which the pruning is applied.
        

    %\item \textbf{Guaranteed Sparsity Level after Pruning Era} (see~\ref{sec:layer-pruning} for more information on \textit{sparsity level}). 
    %Some networks don't guarantee a certain sparsity level as they do not have a strict parameter budget when they prune. They only prune weights that appear to be irrelevant and not with a specific compression goal.
    \item \textbf{Strictness of Parameter Budget Era wrt to Pruning}:
    A strict parameter budget is fixed to the size of the final sparse model. Mostafa and Wang \cite{mostafa2019parameter} have a strict budget throughout training. Our method is only strict after the pruning era. 
    Some networks do not have a strict parameter budget and only prune weights that appear to be irrelevant and without a sparsity target. %\TODO{change its name} Note: the reason this was changed because we don't have sparsity in the first 20 epochs and then end epochs, Note 2: changed it back to strict blah blah
    
    \item \textbf{Pruning Granularity}: The level of granularity within in the network at which values are pruned.  For example, at the kernel level we determine which values to prune by examining only the weights in the kernel \cite{mao2017exploring}. See Figure~\ref{fig:3x3convprune} for more information. 
    


    

\end{enumerate}
\begin{table}
\vspace{0pt}
\centering
\footnotesize

\begin{tabular}{|c|c|c|c|c|c|}
    \hline
\begin{comment}
\thead{Method}                                                  & \thead{Train/\\ Comprss \\ Focus}& \thead{Requires \\ Regular}        & \thead{Strict \\ Parameter \\ Budget \\ Era} & \thead{Granularity\\of Sparsity}  & \thead{Pruning \\ Era}
\\ \hline
 Window Pruning (This Work)                                     & T                                 & No                                & After Pruning                                 & non-structured                    & Beginning      \\
 CK/Combined Pruning (This Work)                             & T                                 & No                                & After Pruning                                 & Kernel                            & Middle      \\
 Sparse Evolutionary Training \cite{mocanu2018scalable}         & T                                 & No                                & Throughout                                    & non-structured                    & Beginning        \\
 tf.contrib.model\_pruning \cite{topruneornot}                  & T                                 & No                                & After Pruning                                 & non-structured                    & Through\\
   Lottery Ticket \cite{frankle2018lottery}                      & T                                 & No                                & Throughout                                   & non-structured                             & Through       \\
  RNN Pruning \cite{narang2017exploring}                        & T                                 & No                                & None                                          & non-structured                    & Beginning  \\
  NN Synthesis Tool (NeST)\cite{dai2017nest}                    & T                                 & No                                & None                                          & non-structured                    & Through\\
   \hline
 PruneTrain \cite{prunetrain}                                   & T                                 & Yes                               & After Pruning                                 & Layer/Channel                     & Through \\
 Dynamic Sparse \cite{mostafa2019parameter}                     & T                                 & Yes                               & Throughout                                    & non-/Kernel                             & Through\\
 Deep Rewiring (DeepR) \cite{DBLP:journals/corr/abs-1711-05136} & T                                 & Yes                               & Throughout                                    & non-structured                    & Through\\
 \hline
 \hline
 Deep Comp \cite{han2015deep,han2015learning}             & C                                 & No                                & -                                             & non-structured                    & Through\\
 \hline
 L1-Norm Channel Pruning * \cite{li2016pruning}                 & C                                 &Yes                                & -                                             & Channel                           &Through\\
 Group-wise Brain Dmg \cite{lebedev2016fast}                    & C                                 & Yes                               & -                                             & non-structured                    & End       \\
 Sparsity Granularity \cite{mao2017exploring}                   & C                                 & Yes                               & -                                              & non-structured                    & Through  \\
SSL \cite{wen2016learning}                                      & C                                 & Yes                               & -                                             & Channel/Kernel/Layer              & Through\\
 ThiNet \cite{luo2017thinet}                                    & C                                 & Yes                               & -                                             & Channel                           & End       \\
 LASSO-regression Prun \cite{he2017channel}                     & C                                 & Yes                               & -                                             & Channel                           & End       \\
 Network Slimming \cite{liu2017learning}                        & C                                 & Yes                               & -                                             & Channel                           & Through\\
 Sparse Structure Selection \cite{huang2018data}                & C                                 & Yes                               & -                                             & Layer                             & Through\\
 Principal Filter Analysis (PFA) \cite{suau2018principal}       & C                                 & Yes                               & -                                             & Channel                           & Through\\ \hline
\end{comment}
\thead{Method}                                                  & \thead{Train/\\ Cmprss \\ Focus} & \thead{Requires \\ Regular\\-ization}& \thead{Pruning \\ Era}  & \thead{Strict \\ Parameter \\ Budget \\ Era}  & \thead{Granularity\\of Sparsity}  
\\ \hline
 Window (This Work)                                     & T                                 & No                         & Beginning           	  & After Pruning                                 & non in Window                    	 \\
 CK/Combined (This Work)                             & T                                 & No                         & Middle      			  & After Pruning                                 & Kernel                            	\\
 Evolutionary \cite{mocanu2018scalable}                  & T                                 & No                         & Beginning        	  & Throughout                                    & non-structured                    	\\
 Zhu and Gupta \cite{topruneornot}                                            & T                                 & No                         & Throughout			  & After Pruning                                 & non-structured                    	\\
   Lottery \cite{frankle2018lottery}                      & T                                 & No                        & Throughout             & Throughout                                   & non-structured                        \\
  RNN Pruning \cite{narang2017exploring}                        & T                                 & No                         & Beginning  			  & None                                          & non-structured                    	\\
  NeST\cite{dai2017nest}                    & T                                 & No                         & Throughout			  & None                                          & non-structured                    	\\
  Variational Dropout \cite{molchanov2017variational} & T                                 & No                        & Throughout			  & None                                    & non-structured                    	\\
   \hline
 PruneTrain \cite{prunetrain}                                   & T                                 & Yes                        & Throughout 			  & After Pruning                                 & Layer/Channel                     	\\
 Dyn Sparse \cite{mostafa2019parameter}                     & T                                 & Yes                              & Throughout		  & Throughout                                    & non-/Kernel                       	\\
 DeepR \cite{DBLP:journals/corr/abs-1711-05136} & T                                 & Yes                        & Throughout			  & Throughout                                    & non-structured                    	\\
 %L0 Regularization \cite{louizos2017learning} & T                                 & Yes                        & Throughout			  & None                                    & non-structured                    	\\
 \hline
 \hline
 Deep Comp \cite{han2015learning}             & C                                 & No                         & Throughout			  & -                                             & non-structured                    	\\
 \hline
 L1-Norm Channel \cite{li2016pruning}                 & C                                 &Yes                         &Throughout			  & -                                             & Channel                           	\\
Brain Damage \cite{lebedev2016fast}                        & C                                 & Yes                        & End       			  & -                                             & non-structured                    	\\
 Sparsity Gran \cite{mao2017exploring}                   & C                                 & Yes                         & Throughout  		  & -                                              & non-structured                   	\\
SSL \cite{wen2016learning}                                      & C                                 & Yes                        & Throughout			  & -                                             & Channel/Kernel/Layer              	\\
 ThiNet \cite{luo2017thinet}                                    & C                                 & Yes                        & End       			  & -                                             & Channel                           	\\
 LASSO-regression \cite{he2017channel}                     & C                                 & Yes                        & End       			  & -                                             & Channel                           	\\
 Slimming \cite{liu2017learning}                        & C                                 & Yes                        & Throughout			  & -                                             & Channel                           	\\
 SSS \cite{huang2018data}                & C                                 & Yes                        & Throughout			  & -                                             & Layer                             	\\
 PFA \cite{suau2018principal}                                   & C                                 & Yes                        & Throughout			  & -                                             & Channel                           	\\ 
 \hline


\end{tabular}
\vspace{5pt}
\caption{Comparison of Training Methods that yield sparse networks } \label{tab:sparsity_work}
\vspace{-15pt}

\end{table}



% this table is subsumed by table in the Results section not needed
\begin{comment}
\begin{table}
\centering
\footnotesize
%\scriptsize
\begin{tabular}{|c|c|c|c|c|}
    \hline
\thead{Method} & \thead{Imagenet \\ Top1 Accuracy}& \thead{Imagenet \\ Top5 Accuracy}& \thead{Epochs to \\ Convergence} &\thead{Final Sparsity}
\\ \hline
This Work 
& 74.89\% & 91.99\% & 90 & 58\%   \\
 PruneTrain 
& 74.33\% & NA & 90 & 53\% \\ 
Dynamic Sparse
& 73.3\% & 92.4\% & 100 & 80\% \\
\hline
\end{tabular}
\vspace{5pt}
\caption{Comparison of Model Pruning accuracy for different sparsity mechanisms} \label{tab:sparsity_methods}
\end{table}
\end{comment}


We chose these concepts because their characteristics can enable faster and lower-energy training. 
A strict parameter budget allows the hardware mapping to plan for a fixed number of multiply-accumulate operations \cite{EIE}. 
Moreover, it allows a lower, fixed amount of physical memory to be allocated to an accelerator \cite{sohoni2019low,mostafa2019parameter,golub2018deep}.
The granularity of the sparsity mechanism indicates how easy it is to adapt the mechanism to an existing hardware. 
The coarser the granularity, the more adaptable it is to existing hardware~\cite{mao2017exploring}. 
Regularization, although useful in forcing the network to learn prunable weights, adds more non-linearity (and thus irregularity) to computation flow \cite{wu2018l1}. 
Pruning in the earlier epochs allows us to train with a compressed network for the majority of training. 

Mao et al. \cite{mao2017exploring} explores pruning on a range of granularities including window, kernel, and filter, and their effect on accuracy, using ImageNet on a number of CNN architectures, including ResNet-50, VGG, and GoogLeNet. 
They also qualitatively and quantitatively show that coarse-grain pruning, like kernel- or filter-level sparsity, is more energy-efficient due to fewer memory references.
Similarly, our work surveys sparsity at the window, kernel, and filter levels. We improve on Mao et al.'s work in two ways.
First, we show higher top-5 accuracy at higher sparsity levels on a complex benchmark, ImageNet on ResNet-50 (92.338\% at 40\% CK sparsity), and we also show high top-1 accuracy whereas Mao et al. only report top-5. 

Prunetrain \cite{prunetrain} explores a way to create sparse channels and even layers to speed up training with around a 1\% drop in accuracy. However, this requires a shift in the training mechanism, including a regularization term that could effect how the mechanism scales to large and distributed settings and that must be computed throughout training. 
The resulting network is only around 50\% sparse and the accuracy loss due to sparse training is high enough that a baseline network with same accuracy could result into same computational savings by just terminating training at much earlier stage/epoch. 

Gale et al. \cite{gale2019state} thoroughly characterize variational dropout \cite{molchanov2017variational}, L0-regularization \cite{louizos2017learning}, and Zhu and Gupta's \cite{topruneornot} magnitude-based pruning applied to Transformers and ImageNet on ResNet-50. Using larger batch size (1024) training they are able to achieve high accuracy (within 1\% decrease) compared to their baseline on ResNet-50 with variational dropout and magnitude-based pruning. However, L0-regularization was unable to produce sparsified networks without high loss in accuracy on ResNet-50, and the other two methods provide unstructured sparsity. In contrast, our work fixes the structure of the network early on in training, making our sparse training possible for hardware to accelerate.

In contrast to other pruning mechanisms, our proposed window, CK, and combined sparsity mechanisms have strict parameter budgets after the pruning era. The CK and combined schemes have channel-level and kernel-level pruning granularities.
% From lottery ticket paper: need to rephrase:
%Bellec et al. (2018) train with sparse networks and replace weights that reach zero with new random connections. Srinivas et al. (2017) and Louizos et al. (2018) learn gating variables that minimize the number of nonzero parameters. Narang et al. (2017) integrate magnitudebased pruning into training. Gal & Ghahramani (2016) show that dropout approximates Bayesian inference in Gaussian processes. Bayesian perspectives on dropout learn dropout probabilities during training (Gal et al., 2017; Kingma et al., 2015; Srinivas & Babu, 2016). Techniques that learn perweight, per-unit (Srinivas & Babu, 2016), or structured dropout probabilities naturally (Molchanov et al., 2017; Neklyudov et al., 2017) or explicitly (Louizos et al., 2017; Srinivas & Babu, 2015b) prune and sparsify networks during training as dropout probabilities for some weights reach 1. In contrast, we train networks at least once to find winning tickets. These techniques might also find winning tickets, or, by inducing sparsity, might beneficially interact with our methods.



==> Sparsity Paper (2)/Results.tex <==

\section{Results}
\label{sec:results}

% Here we mention our results for each set of experiments defined above. 

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% TINY IMAGENET %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{ResNet-50 on Tiny-Imagenet}

From our experiments  with Tiny-Imagenet, we see that even with up to 80\% sparsity, both window and CK pruning are able to achieve levels of accuracy comparable to the dense baseline. CK pruning performs even better than the baseline. Our results are shown in Table~\ref{tab:window_ck_resnet50_timagenet} below.


% window + ck resnet 50 tiny imagenet table
\begin{table}[t]
    \vspace{-5pt}
    \centering
    \footnotesize
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
         & \multicolumn{3}{c|}{\thead{Window}} & \multicolumn{3}{c|}{\thead{CK}} \\ \hline
         \thead{Model \\ Sparsity [\%]}& \thead{Accuracy [\%]} & \thead{Epoch of \\Convergence} & \thead{True \\ sparsity} & \thead{Accuracy [\%]} & \thead{Epoch of \\Convergence} & \thead{True sparsity [\%]}\\ \hline
         0 & 52.03 & 40 & 0.01 & 51.84 & 31 & 0.021\\
         20     & 50.97 & 40 & 0.48 & 52.40 & 31 & 0.207 \\
         40     & 51.62 & 39 & 0.58 & 51.79 & 31 & 0.404 \\
         60     & 52.09 & 40 & 0.69 & 52.56 & 31 & 0.602 \\
         80     & 51.16 & 36 & 0.84 & 52.07 & 31 & 0.800 \\ \hline
    \end{tabular}
    \vspace{0pt}
    \caption{Best accuracy for different sparsity levels for ResNet-50 on Tiny-Imagenet with Window and CK Pruning. Both methods see high accuracy close to, or even above the baseline in the cases of Window at 60\%, CK at 20\%, 60\% and 80\%. CK converges to the final epoch at the same epoch as the baseline while window converges at the same epoch or earlier in the cases of 40\% and 60\%.}
    \label{tab:window_ck_resnet50_timagenet}
    \vspace{-5pt}
\end{table}

\begin{comment}
\begin{table}[t]
    \vspace{0pt}
    \centering
    
    \begin{tabular}{|c|c|c|} \hline
         \thead{Model \\ Sparsity [\%]}& \thead{Window \\ Accuracy [\%]}& \thead{CK \\ Accuracy [\%]}\\ \hline
         0      & 52.03 & 51.84 \\
         60     & 52.09 & 52.56 \\
         80     & 51.16 & 52.07 \\ \hline
    \end{tabular}
    \vspace{10pt}
    \caption{Main results for ResNet-50 on Tiny-Imagenet with Window and CK Pruning.}
    \label{tab:main_window_ck_resnet50_timagenet}
    \vspace{0pt}
\end{table}
\end{comment}


\begin{comment}
Our models actually perform better than the baseline with the following configurations: window pruning with 60\% sparsity as well as CK pruning with 20\%, 60\% and 80\% sparsity. The number of epochs required to reach the converge to the final accuracies is the same for CK and earlier for window at 40\% and 60\% sparsity.


% window + ck resnet 50 tiny imagenet table
\begin{table}[H]
    \vspace{-5pt}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|} \hline
         & \multicolumn{3}{c|}{\thead{Window}} & \multicolumn{3}{c|}{\thead{CK}} \\ \hline
         \thead{Model \\ Sparsity [\%]}& \thead{Accuracy [\%]} & \thead{Epoch of \\Convergence} & \thead{True \\ sparsity} & \thead{Accuracy [\%]} & \thead{Epoch of \\Convergence} & \thead{True sparsity [\%]}\\ \hline
         0 & 52.03 & 40 & 0.01 & 51.84 & 31 & 0.021\\
         20     & 50.97 & 40 & 0.48 & 52.40 & 31 & 0.207 \\
         40     & 51.62 & 39 & 0.58 & 51.79 & 31 & 0.404 \\
         60     & 52.09 & 40 & 0.69 & 52.56 & 31 & 0.602 \\
         80     & 51.16 & 36 & 0.84 & 52.07 & 31 & 0.800 \\ \hline
    \end{tabular}
    \vspace{-5pt}
    \caption{Best Accuracy for different sparsity levels for ResNet-50 on Tiny-ImageNet with Window and CK Pruning}
    \label{tab:window_ck_resnet50_timagenet}
    \vspace{-5pt}
\end{table}

\end{comment}

\begin{comment}
% ck resnet 50 tiny imagenet table
\begin{table}[H]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|} \hline
        \thead{Model Sparsity}& \thead{Accuracy} & \thead{Epoch of \\Convergence} & \thead{True sparsity} \\ \hline
         Standard & 51.84\% & 31 & .021 \\
         20\% & 52.40\% & 31 & 0.207 \\
         40\% & 51.79\% & 31 & 0.404 \\
         60\% & 52.56\% & 31 & 0.602 \\
         80\% & 52.07\% & 31 & 0.800 \\ \hline
    \end{tabular}
    \caption{Final accuracies for ResNet-50 on Tiny-ImageNet for CK Pruning}
    \label{tab:ck_resnet50_timagenet}
\end{table}
\end{comment}

%%% 60% Sparsity ResNet-50 v1.5 results
\begin{figure}[t]
    \vspace{0pt}
    \centering
    \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.35\textwidth,
                    height=0.30\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Top-1 Accuracy},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\footnotesize},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\footnotesize},
                    xmax=100,
                    xmin=50,
                    legend pos=south east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]
    \addplot table [x=, y=resnet1_5_50_baseline-dense-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/dense/Val_Prec_1_Avg.csv};
    \addlegendentry{Dense}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-cksparse60-lr0-05-intra-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-window60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Prec_1_Avg.csv};
    \addlegendentry{Window, Start 30}

    \end{axis}
    \end{tikzpicture}
\qquad
\begin{comment}
    \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.45\textwidth,
                    height=0.30\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Top-1 Accuracy},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\small},
                    xmax=100,
                    xmin=50,
                    legend pos=south east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]
    \addplot table [x=, y=resnet1_5_50_baseline-dense-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/dense/Val_Prec_1_Avg.csv};
    \addlegendentry{Dense}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40}
    \addplot table [x=, y=resnet1_5_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40}
    \addplot table [x=, y=resnet1_5_50_baseline-era30-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40_era30/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40, Era 30}
    \addplot table [x=, y=resnet1_5_50_baseline-era30-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40_era30/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40, Era 30}
    
    \end{axis}
    \end{tikzpicture}
\end{comment}
     \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.45\textwidth,
                    height=0.3\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Network Sparsity},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\footnotesize},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\footnotesize},
                    xmax=100,
                    xmin=0,
                    legend pos=outer north east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]
    %\addplot table [x=, y=resnet1_5_50_baseline-dense-lr0-05out.out, col sep=comma]
    %{ck_imagenet_resnet50v1_5/sparse60/dense/Val_Sparsity.csv};
    %\addlegendentry{Dense}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-0-window60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start0/Val_Sparsity.csv};
    \addlegendentry{Window, Start 0}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-20-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start20/Val_Sparsity.csv};
    \addlegendentry{CK, Start 20}
    %\addplot table [x=, y=resnet1_5_50_baseline-epoch-20-cksparse60-lr0-05-intra-out.out, col sep=comma]
    %{ck_imagenet_resnet50v1_5/sparse60/start20/Val_Sparsity.csv};
    %\addlegendentry{Combined, Start 20}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Sparsity.csv};
    \addlegendentry{CK, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-cksparse60-lr0-05-intra-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Sparsity.csv};
    \addlegendentry{Combined, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-window60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Sparsity.csv};
    \addlegendentry{Window, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Sparsity.csv};
    \addlegendentry{CK, Start 40}
    %\addplot table [x=, y=resnet1_5_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    %{ck_imagenet_resnet50v1_5/sparse60/start40/Val_Sparsity.csv};
    %\addlegendentry{Combined, Start 40}
    \addplot table [x=, y=resnet1_5_50_baseline-era30-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40_era30/Val_Sparsity.csv};
    \addlegendentry{CK, Start 40, Era 30}
    \addplot table [x=, y=resnet1_5_50_baseline-era30-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40_era30/Val_Sparsity.csv};
    \addlegendentry{Combined, Start 40, Era 30}
    
    

    \end{axis}
    \end{tikzpicture}
   


%\qquad % <----------------- SPACE BETWEEN PICTURES
    \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.35\textwidth,
                    height=0.30\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Top-1 Accuracy},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\footnotesize},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\footnotesize},
                    xmax=100,
                    xmin=50,
                    legend pos=south east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]
    \addplot table [x=, y=resnet1_5_50_baseline-dense-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/dense/Val_Prec_1_Avg.csv};
    \addlegendentry{Dense}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-20-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start20/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 20}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-30-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start30/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 30}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40}
    
    \end{axis}
    \end{tikzpicture}
\qquad % <-------------
    \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.45\textwidth,
                    height=0.30\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Top-1 Accuracy},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\footnotesize},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\footnotesize},
                    xmin=65,
                    xmax=100,
                    legend pos=outer north east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]

    \addplot table [x=, y=resnet1_5_50_baseline-dense-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/dense/Val_Prec_1_Avg.csv};
    \addlegendentry{Dense}
    \addplot table [x=, y=maxnonzero_4_60_0_30_nofc_mlplr_steps, col sep=comma]
    {imagenet_resnet50_window_sparsity/Val_Prec_1_Avg.csv};
    \addlegendentry{Window, Start 0, v1}
    \addplot table [x=, y=resnet1_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/v1/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40, v1}
    \addplot table [x=, y=resnet1_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/v1/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40, v1}
    
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-0-window60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start0/Val_Prec_1_Avg.csv};
    \addlegendentry{Window, Start 0, v1.5}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40, v1.5}
    \addplot table [x=, y=resnet1_5_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40, v1.5}
    \end{axis}
    \end{tikzpicture}
%\qquad % <----------------- SPACE BETWEEN PICTURES
\vspace{-10pt}
\caption{top left: Convergence plots of all pruning methods with first epoch of pruning 30,
%CK and combined with different pruning era lengths of 20 and 30 (top right),
top right: Sparsity plot of all methods,
bottom left: and CK starting pruning at different epochs,
bottom right: ResNet v1 and v1.5 at 60\% sparsity for 90 epochs.}
\vspace{-10pt}
\label{fig:sparse60_resnet50v15_imagenet}
\end{figure}

%%%%%%%%%%%%%%%%%%%%
%%%%% IMAGENET %%%%%
%%%%%%%%%%%%%%%%%%%%

\subsection{ResNet-50 on Imagenet}


\begin{comment}
On Imagenet, we experimented with transfer learning with kernel pruning. While we do not want to fully train the model and then prune as this would significantly increase the full amount of time required to train, we attempt to train the model dense to an intermediate epoch and introduce sparsity later in training. We tried starting the sparsity from epoch 40 and epoch 20. From these two starting epochs, we tried to prune for to various levels of sparsity 0-60\%. \KK{think this section is already covered in Experimental Setup}.
\end{comment}

Our ResNet-50 v1.5 experiments (Table~\ref{tab:main_results100} and Appendix Figure~\ref{fig:start30_resnet50v15_imagenet}) with the  \textit{first epoch of pruning} at epoch 30 show that all of our pruning methods are able to achieve over 73\% accuracy, and we can achieve above 74\% accuracy up to 70\% sparsity.  

By comparing the sparsity curves of the window, CK, and combined pruning runs in Figure~\ref{fig:sparse60_resnet50v15_imagenet} (top right), we observe that the sparsity of window pruning is not as smooth as the other methods. This is likely indicative of the more rigid structure of CK and combined pruning, which causes the degree of sparsity to be much more uniform from epoch to epoch. 
Figure~\ref{fig:sparse60_resnet50v15_imagenet} (top left, bottom right) also shows on ResNet v1.5, the window is slightly better than the CK and combined, which have similar performance, but the window is worse than the other two on ResNet v1. 
Furthermore, starting the \textit{pruning era} later improves performance (Figure~\ref{fig:sparse60_resnet50v15_imagenet}-(bottom left)).

Table~\ref{tab:main_resnet_v1} shows that on ResNet-50 v1, our methods can achieve between 0.1-0.3\% less than the baseline. 
Here, we do not compare to compression focused methods as they take around 180 epochs of training if aiming for levels of accuracy that reported. If not, they have much worse accuracy numbers without providing structured sparsity and without the potential of computation savings during training.




\begin{comment}
%%% ResNet v1 vs v1.5 comparison at 60%
\begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[cycle list name=tb, 
                    width=0.50\textwidth,
                    height=0.40\textwidth,
                    grid=both,
                    grid style={solid,gray!30!white},
                    axis lines=middle,
                    xlabel={Epoch},
                    ylabel={Accuracy},
                    x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
                    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south,font=\small},
                    xmin=40,
                    xmax=90,
                    legend pos=outer north east,
                    tick label style={font=\tiny},
                    legend style={font=\tiny}
                    ]

    \addplot table [x=, y=maxnonzero_4_60_0_30_nofc_mlplr_steps, col sep=comma]
    {imagenet_resnet50_window_sparsity/Val_Prec_1_Avg.csv};
    \addlegendentry{Window, Start 0, v1}
    \addplot table [x=, y=resnet1_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/v1/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40, v1}
    \addplot table [x=, y=resnet1_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/v1/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40, v1}
    
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-0-window60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start0/Val_Prec_1_Avg.csv};
    \addlegendentry{Window, Start 0, v1.5}
    \addplot table [x=, y=resnet1_5_50_baseline-epoch-40-cksparse60-lr0-05out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{CK, Start 40, v1.5}
    \addplot table [x=, y=resnet1_5_50_baseline-lr05-epoch-40-intra-combo-cksparse60-out.out, col sep=comma]
    {ck_imagenet_resnet50v1_5/sparse60/start40/Val_Prec_1_Avg.csv};
    \addlegendentry{Combined, Start 40, v1.5}
    \end{axis}
    \end{tikzpicture}
\vspace{-10pt}
\caption{Comparison between ResNet v1 and v1.5 at 60\% sparsity after 90 epochs}
\label{fig:resnet50_v1_vs_v15}
\end{figure}

By comparing tables \ref{tab:main_results100} and \ref{tab:main_results90}, we can observe that the final 10 epochs of training after the learning rate drop at epoch 90 are very important for accuracy as they can achieve a gain of 0.7-1.1\%.


\end{comment}


%%% Start Final Results Tables
\begin{table}[t]
    %\footnotesize
    \vspace{0pt}
    \centering
    \begin{tabular}{|c|c|c|c|c|} \hline
    Model Sparsity (\%) & 40 & 60 & 70 & 80 \\ \hline \hline
    Dense (76.29) & - & - & - & - \\ \hline
    CK, start 40 & 75.82 (-0.46) & 75.33 (-0.95) & 74.92 (-1.36) & \textbf{74.16 (-2.12)} \\
    CK, start 30 & 75.84 (-0.45) & 75.12 (-1.17) & 74.72 (-1.56) & 73.66 (-2.63) \\
    CK, start 20 & 75.55 (-0.74) & 74.71 (-1.58) & 74.32 (-1.96) & 72.79 (-3.50) \\ \hline
    Combined, start 40 & \textbf{75.89 (-0.39)} & \textbf{75.38 (-0.90)} & \textbf{75.07 (-1.21)} & 74.02 (-2.27)\\ 
    Combined, start 30 & 75.84 (-0.45) & 75.16 (-1.12) & 74.48 (-1.80) & 73.66 (-2.63) \\ 
    Combined, start 20 & 75.72 (-0.57) & 74.75 (-1.53) & 74.26 (-2.02) & 72.97 (-3.32) \\ \hline
    Window, start 0 & - & 73.63 (-2.65) & 72.79 (-3.50) & 70.25 (-6.04) \\ 
    Window, start 30 & - & 75.45 (-0.84) & 74.65 (-1.63) & 73.31 (-2.98) \\ \hline
    CK, start 40, era 40-70    & - & 75.52 (-0.77) & \textbf{75.16 (-1.13)} & - \\
    Combined, start 40, era 40-70 & - & \textbf{75.56 (-0.73)} & 75.14 (-1.15) & - \\ \hline
    \end{tabular}
    \vspace{5pt}
    \caption{Main results, top-1 accuracy on ResNet-50 v$1.5$ after 100 epochs.}
    \vspace{-10pt}
    \label{tab:main_results100}
\end{table}


\begin{table}[t]
    %\footnotesize
    \centering
    \begin{tabular}{|c|c|c|c|c|} \hline
    Model Sparsity (\%) & 40 & 60 & 70 & 80 \\ \hline \hline
    Dense (75.25) & - & - & - & - \\ \hline
    CK, start 40 & 74.93 (-0.32) & 74.6 (-0.65) & 74.21 (-1.04) & \textbf{73.34 (-1.91)} \\
    CK, start 30 & \textbf{74.96 (-0.29)} & 74.25 (-1.00) & 73.83 (-1.42) & - \\
    CK, start 20 & 74.74 (-0.51) & 73.84 (-1.41) & 73.37 (-1.88) & 72.49 (-2.76) \\ \hline
    Combined, start 40 & 74.91 (-0.34) & \textbf{74.75 (-0.50)} & \textbf{74.36 (0.89)} & 73.22 (-2.03) \\ 
    Combined, start 30 & 74.94 (-0.31) & 74.41 (-0.84) & 73.87 (-1.38) & - \\ 
    Combined, start 20 & 74.73 (-0.52) & 73.65 (-1.60) & - & 72.22 (-3.03) \\ \hline
    Window, start 0 & - & 72.63 (-2.62) & 71.79 (-3.46) & 69.48 (-5.77) \\ 
    Window, start 30 & - & 74.28 (-0.97) & 73.88 (-1.37) & 72.63 (-2.62) \\ \hline
    CK, start 40, era 40-70    & - & 74.67 (-0.58) & 74.34 (-0.91) & - \\
    Combined, start 40, era 40-70 & - & \textbf{74.77 (-0.48)} & \textbf{74.38 (-0.87)} & - \\ \hline
    \end{tabular}
    \vspace{5pt}
    \caption{Main results, top-1 accuracy on ResNet-50 v$1.5$ after 90 epochs.}
    \label{tab:main_results90}
\end{table}




% ResNet-50 v1 and comparison to other works
\begin{table}[!t]
    \footnotesize
    \vspace{-10pt}
    \centering
    \begin{tabular}{|c||c|c||c|c||} \hline
    & \multicolumn{2}{c||}{Epoch 90} & \multicolumn{2}{c||}{Epoch 100} \\ \hline
    Model & Sparsity [\%] & Accuracy [\%] & Sparsity [\%] & Accuracy [\%] \\ \hline \hline
    CK, start 40    & 60 & 74.60 & 60 & 75.36 \\
    Combined, start 40 & 60 & 74.68 & 60 & 75.37 \\
    Window, start 0 & 60 & 74.78 & - & - \\
    CK, start 30 & - & - & 80 & 73.66  \\ \hline
    %PruneTrain (\cite{prunetrain})           & 0.53 & -1.87 & - & - \\
    %Dyn Sparse (\cite{mostafa2019parameter}) & - & - & 0.80 & -1.60 \\ \hline
    PruneTrain (\cite{prunetrain})           & 50 & 73.0 & - & - \\
    Dyn Sparse (\cite{mostafa2019parameter}) & - & - & 80 & 73.3 \\ 
    Dyn Sparse (kernel granularity) & - & - & 80 & 72.6 \\\hline
    \end{tabular}
    \vspace{5pt}
    \caption{Main results, top-1 accuracy on ResNet-50 v1 after 90 and 100 epochs. Comparison with related work. PruneTrain sparsity is not explicitly stated, so we estimate their sparsity level from their inference FLOPs saved (1-FLOPs). Also, our experiments were run with batch size 64.}
    \vspace{-10pt}
    \label{tab:main_resnet_v1}
\end{table}

%We also experimented with moving the learning rate drop at epoch 90 to epoch 80, but according to Appendix Table~\ref{tab:drop80} and Table~\ref{tab:main_results100} the improvement is marginal.

\begin{comment}

%\begin{wraptable}{r}{5.5cm}
\begin{table}[H]
    \centering
    \footnotesize
    \begin{tabular}{|c|c|} \hline
    Experiment @ 60\% Sparsity & Accuracy (Improvement) [\%] \\ \hline \hline
    CK, start 40 & 75.39 (0.05) \\
    CK, start 30 & 75.06 (-0.06)\\
    CK, start 20 & 74.80 (0.09)\\ \hline
    Combined, start 40 & 75.46 (0.08) \\
    Combined, start 30 & 75.19 (0.03) \\
    Combined, start 20 & 74.88 (0.13) \\ \hline
    Window, start 0 & 73.89 (0.26) \\ \hline
    \end{tabular}
    \caption{Results when we changed final learning rate drop from epoch 90 to 80, top-1 accuracy on ResNet-50 v$1.5$ at epoch 100. \AP{this should go to Appendix. In text mention in one sentence the conclusion}}
    \label{tab:drop80}
\end{table}
%\end{wraptable}
%%% End Final Results Tables
\end{comment}

\begin{figure}[t]
    \centering
    \vspace{0pt}
    \includegraphics[width= .95 \textwidth]{Figures/Layer_Sp.pdf}
    \vspace{-5pt}
    \caption{ResNet-50 v1.5 layer sparsity for CK, start 30, targetting 70\% sparsity.}
    \vspace{-5pt}
    \label{fig:Layer_sp}
\end{figure}






 Table~\ref{tab:window_resnet50_imagenet_adversarial} demonstrates that our sparsity mechanism can have a minimal drop in adversarial robustness (approximately 1-1.5\%) compared to the dense baseline model, whereas other methods see more accuracy degradation \cite{wang2018adv}. %All pruning methods perform fairly consistently with each other at 60\% and 70\% sparsity.

The sparsity of each layer, depicted in Figure~\ref{fig:Layer_sp}, emphasizes that early layers tolerate sparsity better, as they have consistently higher sparsity in the last 1$\times$1 convolutional layer of each residual block. This may be due to their vicinity to the residual connection, which provides additional information to the layer. 

Table \ref{tab:batch256_table} shows the results for select experiments with batch 256, which reflects more typical ResNet training. 

%%% Start Final Batch 256 Results Tables
\begin{table}[t]
    
    \vspace{0pt}
    \centering
    \begin{tabular}{|c|c|c|} \hline
    Model Sparsity (\%) & 60 & 70 \\ \hline \hline
    Dense (76.53) & - & - \\ \hline
    CK, start 20 & - & 74.72 (-1.81) \\
    CK, start 30 & - & \textbf{75.13 (-1.40)} \\ \hline
    Window, start 20 & - & 74.68 (-1.85) \\
    Window, start 30 & - & 74.87 (-1.66) \\
    Window, start 40 & - & 75.03 (-1.50) \\ 
    Window, start 0, era 0-30 & 73.95 (-2.58) & - \\ \hline
    Combined, start 20 & - & 74.01 (-2.52) \\
    Combined, start 30 & - & 74.44 (-2.09) \\
    Combined, start 40 & - & 74.62 (-1.91) \\ \hline
    \end{tabular}
    \vspace{5pt}
    \caption{Main results, top-1 accuracy on ResNet-50 v1 after 100 epochs, using batch size 256.}
    \vspace{0pt}
    \label{tab:batch256_table}
\end{table}

% Adversarial robustness, window
\begin{table}[!ht]
    \vspace{0pt}
    %\footnotesize
    \centering
    \begin{tabular}{|c |c | c|c|c|c|c|c|} \hline
         Model & Sparsity & \(\epsilon= .05\)& \(\epsilon=.1\) & \(\epsilon = .15\) & \(\epsilon=.2\) & \(\epsilon=.25\) & \(\epsilon=.3\)  \\ \hline
         %Dense & 40.37\% & 28.84\% & 23.33\% & 20.25\% & 18.34\% & 17.08\% \\
         %60\% & 38.9\% & 27.17\% & 21.48\% & 18.21\% & 16.16\% & 14.78\% \\ 
         %80\% & - & - & - & - & - & - \\ \hline
         Dense & 0 & 41.71 & 30.47 & 25.24 & 22.39 & 20.69 & 19.58 \\
         Combined, start 40 & 0.6 & 40.42 & 29.02 & 23.67 & 20.73 & 18.93 & 17.73 \\
         Combined, start 40 & 0.7 & 40.03 & 28.55 & 23.13 & 20.13 & 18.32 & 17.10 \\
         Window, start 30 & 0.6 & 40.52 & 29.12 & 23.77 & 20.81 & 18.99 & 17.78 \\
         Window, start 30 & 0.7 & 39.73 & 28.32 & 22.91 & 19.88 & 18.02 & 16.77 \\
         CK, start 40 & 0.6 & 40.51 & 29.21 & 23.95 & 21.08 & 19.34 & 18.18 \\
         CK, start 30 & 0.7 & 39.83 & 28.44 & 23.09 & 20.11 & 18.31 & 17.12 \\ \hline
    \end{tabular}
    \vspace{5pt}
    \caption{Adversarial Robustness of ResNet-50 v1.5 on Imagenet}
     \vspace{0pt}
    \label{tab:window_resnet50_imagenet_adversarial}
\end{table}



\subsection{Discussion}

Overall, we notice that there is a tolerance for sparsity (up to 70\%), which yields around 1\% accuracy loss compared to the dense baseline. However, this loss can be compensated by dropping the learning rate and performing another 10 epochs of training, which provides a 0.7-0.9\% accuracy increase. With high levels of sparsity this extension is computationally cheap.

We observed the early stages of dense training are important for high accuracy, as longer periods of dense training consistently outperformed shorter ones.
Moreover, widening the pruning era slightly (10 epochs) improves the final convergence accuracy (by around 0.2\%).

We also observed that pushing the learning rate drop schedule to earlier epochs or aligning it with pruning era does not improve the final accuracy. However, pushing the last learning rate drop from epoch 90 to 80 can improve the accuracy by around 0.1\% (See Appendix Table~\ref{tab:drop80} and Table~\ref{tab:main_results100}).

We postulate that window pruning performs worse for ResNet v1.5 compared to ResNet v1 due to the strided nature of convolutions in ResNet v1.5.

\begin{comment}

%\item there is tolerance to sparsity til 60\%, best is 1\% loss starting epoch 40 for both combined and ck

\item width of the pruning era should be 20 not 30 (shows sensitivity) - TODO need one more data point

\item 

\item pruning can be restricted to small period TODO: wait for last runs to see if (4) holds, but i still think this is true

\item sparse training w/o any modification to network structure/regularization after pruning period, no new pruning either

\item hypothesis: pushing lr drops earlier is not better -> this is true,

\item hypothesis: aligning first lr drop with pruning era is important -> compare 20,50,80 run at each 20 vs 30,60,90 at epoch 30, these results show the former is worse: Not true

\item pushing to last lr drop from 90 to 80 doesn’t help, so try to push the whole schedule -> helps around 0.1%

\item 

\item for coarse grained structured, you need epochs of dense, but for fine grained window pruning, still can prune from 0 without loss of accuracy -> TODO doesnt hold in resent 1.5 (strided convolution hurts)

\item hypothesis: fixing (putting a cap on) the number of maxnonzero values in combined helps -> does not hold, it was worse

\item CK and combo seem to have the same performance between the two network versions even though window is worse on ResNet v1.5. One possible explanation for this is that because ResNet v1.5 uses stride convolutions, fine-grained window sparsity has some effect on the accuracy, but because CK and combo do coarser pruning of whole kernels, the fact that there’s striding doesn’t matter 

\item Widening the pruning era from 40-60 to 40-70 (ie push the end out further) leads to ~0.2 increase in CK

\end{comment}




==> Sparsity Paper (2)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

